Rambler: Supporting Writing With Speech via LLM-Assisted Gist Manipulation

Dictation enables efficient text input on mobile devices. However, writing with speech can produce disfluent, wordy, and incoherent text and thus requires heavy post-processing. This paper presents Rambler, an LLM-powered graphical user interface that supports gist-level manipulation of dictated text with two main sets of functions: gist extraction and macro revision. Gist extraction generates keywords and summaries as anchors to support the review and interaction with spoken text. LLM-assisted macro revisions allow users to respeak, split, merge and transform dictated text without specifying precise editing locations. Together they pave the way for interactive dictation and revision that help close gaps between spontaneous spoken words and well-structured writing. In a comparative study with 12 participants performing verbal composition tasks, Rambler outperformed the baseline of a speech-to-text editor + ChatGPT, as it better facilitates iterative revisions with enhanced user control over the content while supporting surprisingly diverse user strategies.

==> reference/old-content.tex <==
% \michael{I like this intro, for it contains all the important information. But I feel that the current version is too lengthy. Some of the content can be moved to later sections. It would be better if we can use a few paragraphs, each  to directly point out 1) the need of the research, 2) the limitation of the related work, 3) how the proposed method can fill this gap, and 4) some important founding in results and 5) a summary of contribution. This may sounds stereotype, but it gives a clear view and easy to follow. Just as a stepping stone for future revision: }

% \canl{Quoting JD's comment in Slack "we might want to follow a similar framing to Michael's, but point out that there's an existing line of great work around summarization and gist-based interfaces (a term I think we can still coin!) that we think could apply to this critical domain of dictation.
% Then instead of defending our choice of "dictation" as being because spoken text is inherently more fluid and lower stakes than written text, we can point to the proliferation of smartphones and tablets -- and say that dictation is receiving a ton of research interest because the hardware limitations of those devices make existing text authoring tools suboptimal. (And also, spoken text is different from written text.)
% So, we built RambleTool as a design probe to understand how gist-based editing can assist in these mobile/tablet environments where we stand to benefit from voice as primary text input method (vs. character input methods)."}

% \canl{Then I added the following before reading Michael's version: "I agree with starting with the proliferation of mobile platforms with the development of Ubiquitous Computing. From smartphone, tablet to smart glasses and AR/VR goggles, users’ input precision drastically reduce, while existing text authoring interfaces all require too much precision. (Is this a good argument for your point about they are suboptimal? Any other arguments in mind?)}

% \canl{Then the breakthroughs of ASR and NLP being enabling technologies to potentially allow speech becoming a primary text input method. Yet, speech is fundamentally different from writing in terms of its cognitive characteristics, thus produces different outcomes [my CSCW and CUI papers show these], including: much more text produced (a good thing that lowers composition barrier), disfluency and disorganization.}

% \canl{So we built RambleBoxes to …. <Quote JD’s nice phrasing>…
% RambleBoxes(name ideas?) leverages LLM to assist the macro-revision as to clean disfluencies, generating summaries for reviewing and semantically segment and merge text into smooth writings, etc. Different from the obvious conversational interfaces for LLMs, it embeds LLM capabilities behind the GUI tailored for interacting with spoken text. Our study evaluates this approach against the state-of-the-art dictation interface with ChatGPT provided as a side tool.}

% \canl{Contributions include: 1) RambleBoxes - an LLM-assisted novel dictation interface that supports iterative drafting and non-linear composition; 2) Empirical study comparing two types of LLM-powered interface support for reviewing and interacting with spoken text: LLM-powered GUI versus the conversational LLM. "}

% \canl{More from JD:"I think the framing question is whether we want to tout the benefits of speech in general vs. pointing out that speech is ideal for small screens and form factors without hardware keyboards.
% I’d say that existing/traditional text authoring interfaces are not ideal because:
% 1) Yeah, they require too much precision, like pointing to individual words or even letters.
% 2) They only show you the full character-level text, which may be intractably long or hard to navigate on a small screen.
% 3) They treat dictation input verbatim, mixing spoken and written language in a manner that practically requires revision, which is then hard to do.
% I think I was merely trying to point out that we have multiple avenues for getting people excited about the work, depending a bit on who we want/expect to review our paper. An abstract focused on building upon gist-based user interfaces (like the “Beyond Text Generation” UI) and adapting them to apply to small-form-factor speech-input-focused text authoring and revision could get a pretty broad swath of potential reviewers excited. 
% }

% \michael{Can, thanks for summarizing the discussions on Slack. Also, JD made some good points. I agree that framing the problem toward speech input on mobile devices probably can make the study easier to justify and evaluate.}

% Traditional writing, using pen or typewriter, requires writers to formulate their ideas clearly in mind before committing them to paper. This mindset also affects typing behavior with modern devices, and it may cause hesitation, procrastination, and thus inefficiency in writing. In contrast, starting with a rough idea and iterating on it can be more effective. This process is more natural in speech, especially through ``rambling''. Rambling is a way to express a series of thoughts or ideas, which may be disorganized but can still contain all the important messages.

% The challenge of converting rambling thoughts to written text is to identify the important information then refine and organize it in a logical way. This can be time-consuming and difficult conventionally but greatly simplified by large language models (LLMs) nowadays. That said, the pervasive LLM-based text composing work focuses on text generation [cites] and style transfer [cites]. To the best of our knowledge, little research has studied how to help users quickly review [cite summarization/] and interact [cite redictate \& ai writing tool] with the generated text. None of them has accounted for the both factors to support writing through rambling thoughts. 

% To fill this gap, this paper discusses a novel writing tool (\systemnamenospace) with two important features: semantic zooming and macro revision. \textit{Semantic zooming} aims to support users in efficiently consuming the generated text, by providing different levels of gists. Since LLM can greatly reduce the user workload in refining their rambling thoughts, especially disfluencies [cite], the new productivity bottlenecks become how well users can review, comprehend, and process the generated text. Cognitive science shows that humans remember the gist of words, rather than the exact verbatim. With this in mind, semantic zooming provides multiple levels of summarization of a ramble, and users can adjust the display granularity on the fly. This allows users to reduce the cognitive load to review the LLM output and control their level of attention to each ramble on demand, and encourages them to focus on macro revision.

% \textit{Macro revision} is the process of manipulating text at the sentence level, such as splitting, reorganizing, and merging blocks of text. While LLMs are good at refining and cleaning up ramble scripts, the results may still be poorly structured or misaligned with users' thought processes. However, rearranging text is not trivial. First, users need to review a big chunk of text and identify the proper semantic segmentation. Second, text manipulation, such as precise selection, can be difficult due to the input device and modality, such as the fat finger problem on smartphones. To address this, \systemnamenospace  offers two text segmentation methods. Users can either split the text by specifying the keywords in each block or use an LLM-powered segmentation method. Each ramble box supports direct manipulation. Users can drag and drop them to form a more logical paragraph. Merging the ramble boxes is also powered by LLMs to achieve a coherent result.

% Talk about the important results in experiments.

% Our contribution is three-fold. ...

% \michael{prior version is kept here:}

% The rapid advancement of Speech-To-Text for input and the power of large language models (LLMs) for text generation are reshaping how people write by significantly reducing the barrier of text composition. New productivity bottlenecks in writing are instead in the capacity and efficiency with which users can review, comprehend, and process the abundant text generated with these technologies. 

% Speaking is a more natural, accessible, and fast way to compose than typing or writing <>. As it is a hands-free (and eyes-free) input modality, it is not only useful as an input modality in assistive technology, but it also makes it easier to input text in situations where it is inconvenient to use their hands or eyes: people currently often compose or ideate on small mobile devices where they can’t take advantage of a mechanical keyboard. 

% Yet human speech is much more organic and freeform than typing or writing; for the average person, speech is plagued by both disfluencies, such as long pauses or filler words, and a more non-linear nature, such as repeating or circling back to previously stated ideas <>. Automatic speech transcription often needs manual editing and revision, hindering user adoption of speech as a primary text input method. Prior research in editing for STT has often focused on different modalities for more fine-grained editing, such as redictation for correction, and/or utilizing gaze to select editing targets <>. But since speech input inherently generates more text, traditional fine-grained editing can become incredibly tedious.


% Coincidentally, the recent rise of LLMs has also enabled a much wider, open-ended space of larger-scale text manipulation, which includes the ability to support this kind of conceptual, higher level editing. Previous work has explored the development of AI-human collaborative writing tools – utilizing LLM’s to support writing at varying levels of detail, from word level corrections to suggesting plot points or providing multi-sensory inspiration.

%  Beyond their generative text abilities, LLMs can organize and summarize user text. However, existing LLM platforms like Bard or ChatGPT generally provide chat-style interfaces that only provide users with a narrow, highly structured means of engaging with their text. Recent research has supported cleaning and organizing audio transcripts to provide summaries. For instance, Li et al. explored hierarchical summarization for text transcriptions of verbal discussions with semantic segmentation and merging algorithms [2]. Other recent work [2] investigated using continuous text summarization to help writers reflect on their writing by placing sidebars of summaries that update in real-time with the word processing. While this line of work shows promising results, the domain of support for live speech remains underexplored.


% Users need better controls and visualizations for the iterative process of generating and manipulating text, compared to a default chat-style conversational UI (e.g., Bard, ChatGPT) or with a single-pass summary. While word processing has always featured character-level precision, writing interfaces lack support for coarse-grained text manipulation in larger chunks, potentially limiting users’ productivity. Live speech as a text input modality presents an exciting new set of possibilities yet to be explored. 

% Cognitive science research shows that human memory of text operates by extracting the gist of words instead of remembering the exact verbatim word trace. We seek modern alternatives of interface solutions from simply showing the live, verbatim transcript of what was spoken by a user to higher-level representations that focus more on the text’s gist. The goal is to (a) improve readers’ understanding of what was said and (b) provide augmented ways to edit spoken text. This work will allow users to review spoken text at a higher level with dynamic topic modeling and selectively ‘drill down’ into topics as they like. 

% We plan to build a new dictation and word processing interface powered by LLMs that shows a real-time gist-level visualization of live spoken text. This interface will allow users to control the abstraction level of summarization by supporting smooth semantic zooming within the text, providing visual continuity across different summarization levels. To do this, we will customize the text summarization method by preserving information points that support memorization based on theories in cognitive science across layers of gist extraction. The interface will support coarse-grained text manipulation on the gist level while maintaining references to the original verbatim composition. Based on the initial investigation of user needs, we will iteratively build prototypes using Google Cloud’s Speech API for real-time speech recognition and perform prompt engineering for customized live text summarization. We will evaluate our approaches’ effectiveness in supporting iterative and non-linear verbal drafting as a new way of writing, making one’s spoken composition easier to read and modify. We will also seek to learn how users may adopt new composition and revision strategies with speech input, how graphical interfaces can better support them, and the adaptability of LLMs to support different users with varying style preferences and goals.
% Motivated by the unique characteristics of human speech input, and bolstered by the rise of intelligent text processing in LLMs, we propose a novel web-based speech interface we call the Ramble Tool. Users are encouraged to focus on the bigger picture, as the LLM handles most of the fine-grained editing. We aim for Ramble Tool to redefine the workflow of STT, as mainstream STT interfaces often rely heavily on traditional editing workflows that restrict the inherent benefits of STT. 
% Ramble Tool focuses on supporting iterative drafting and non-linear composition – users of our tool are encouraged to compose primarily through speech, and edit primarily at a more conceptual level, which we term “macro-revisions”. Ramble Tool provides various functionalities that operate on either the level of a whole composition, or on user-specified sections of the composition we term “rambles”: these macro-revisions include creating or deleting a “ramble”, respeaking, semantic zooming, merging, splitting, and reorganizing. Traditional “micro-revisions” that operate on a word or character level are still supported through manual keyboard editing.
% We center our evaluation on exploring how participants adjust to this new mental model of editing and workflow for composition. To evaluate our Ramble Tool, we conducted a within-subjects comparative study (N=12). We evaluated two techniques all based on Ramble Tool: the first condition (Text Editor) only allows dictation and keyboard editing; the second condition condition (LLM-Assisted Rambling) adds on manual and LLM-assisted macro-revision functionalities. Participants are given an iPad and instructed to use each technique to create a composition for a given writing task. 

% <include results once we have>

